Liveness Verification and Synthesis: New Algorithms for Recursive Programs

We consider the problems of liveness verification and liveness synthesis for recursive programs. The liveness verification problem (LVP) is to decide whether a given omega-context-free language is contained in a given omega-regular language. The liveness synthesis problem (LSP) is to compute a strategy so that a given omega-context-free game, when played along the strategy, is guaranteed to derive a word in a given omega-regular language. The problems are known to be EXPTIME-complete and EXPTIME-complete, respectively. Our contributions are new algorithms with optimal time complexity. For LVP, we generalize recent lasso-finding algorithms (also known as Ramsey-based algorithms) from finite to recursive programs. For LSP, we generalize a recent summary-based algorithm from finite to infinite words. Lasso finding and summaries have proven to be efficient in a number of implementations for the finite state and finite word setting.

==> content/introduction.tex <==
\section{Introduction}

TODO.

%    It is well known that context-free grammars can be used to describe the behavior of recursive programs. A rule of type $X \rightarrow a \ | \  YX$ can be interpreted as "procedure $X$ either executes command $a$ or calls procedure $Y$ and does a recursive call of itself afterwards". Therefore, properties of executions of recursive programs can be formulated as properties of the words in the language given by a context-free grammar.\\
%    
%    Liveness verification deals with properties which can be disproved by giving an infinite execution violating the property. To do liveness verification for recursive-programs, we will have to define the language $L^\omega(G)$ of infinite words given by a context-free grammar $G$. Checking whether a liveness property holds then amounts to checking whether the inclusion $L^\omega(G) \subseteq L^\omega(A)$ holds, where $A$ is a Buechi automaton which accepts if the property is fulfilled.\\
%    
%    The first contribution of this paper is an exact definition of the $\omega$-language of a context-free grammar together with a nice representation for such $\omega$-languages obtained from a graph representing the $\omega$-structure of the grammar.\\
%    
%    The second contribution is a decision procedure for the inclusion. It combines and extends techniques from two  related problems:
%    
%    It uses the techniques presented in \cite{meyer_antichainsrecursiveprogverification} to get a finite description of the behavior induced by a (possibly infinitely large) sets of words on an automaton by sets of state transition boxes and extends these to also respect the final states of the automaton.
%    
%    Afterwards, the lasso finding test used to decide $L^\omega(A) \subseteq L^\omega(B)$ for Buechi automata $A, B$ (see \cite{holik_simulationsubsumptionramseybuechi}) is modified such that it can be used to decide $L^\omega(G) \subseteq L^\omega(A)$.


==> content/parity.tex <==
\section{Parity Game Construction}

\subsection{Intuition}

%To the end of an alternative construction from the trees $T_0,...,T_n$, it is also possible to code the choice functions of the prover into the game automaton $A_{game}$, instead of iterating over all possible functions. This automaton will be again be a game arena for prover and refuter.\\

Let us now consider $\sigma$ = sol($S_{inf}$). If $\sigma = \ifalse$, prover can either enforce the derivation of a finite word or of a left-infinite word and wins trivially.
Otherwise, we may assume $\sigma$ to be in conjunctive normal form, i.e. $\sigma = \set{C_1, C_2,...,C_n}$ with non-empty clauses $C_i \subseteq \mathcal{P}(M_A \times N)$.
Intuitively, the play played from $S$ collapses to a game with just two steps:
Prover chooses one of the clauses and refuter chooses one element in this clause.

Actually, we will formalize this the the other way around:
Refuter chooses one element of each clause (we will call this choice "choice function" $c: N \rightarrow \mathcal{P}(N \times M_A$)) and prover picks one of those.
The resulting element is of form $\tbox{w}g.\hat{X}$.
This encoding has algorithmic benefits, since it will be sufficient to store the image of the choice function as a set of tuples in $M_A \times N$.

In terms of games, this means that starting from start symbol S, we derived a word $w' \in \tbox{w}$ during a finite game and need to continue deriving using non-terminal X on the right. Therefore, we now consider sol($X_{inf}$) and continue the process again.

This whole process can be modeled as a bipartite graph $B$:

\begin{enumerate}
    \item
    The node set is partitioned into two different types of nodes $V_{\square}$ and $V_{\roundss}$, which are owned by the players prover and refuter respectively.
    \item
    The graph is bipartite as refuter first chooses the choice function and subsequently prover chooses one element $\tbox{w}.\hat{X}$ contained in the image of the choice function.
    Thus edges span only between nodes of different type.
    \item 
    The nodes $V_{\roundss}$ are labeled by non-terminals.
    From node $X$ in $V_{\roundss}$, prover can choose which choice function (or rather image) he wants to use for formula $X_{inf}$ (this time, he may make another choice if node X is reached again).
    Thus the nodes $V_{\square}$ of prover are labeled by the images of all possible choice functions for that formula.
    From each of these nodes, prover can choose which element from the image will be picked and thus which word (or rather box) will be derived and which non-terminal will be reached at the right.
\end{enumerate}


\subsection{Formal Construction of graph B}

Formally, we have the following construction:
\begin{enumerate}
    \item
    $V = V_\roundss \dotcup V_\square$, where $V_{\roundss}$ = N, $V_{\square}$ = $2^{M_A \times N}$.
    \item
    There is an (unlabeled) edge from node $X \in V_{\roundss}$ to node $C \in V_{\square}$, if C is a valid image of a choice function for non-terminal $X$ (meaning it contains at least one element from each clause and each element in the image is contained in at least one clause).
    \item
    There is an edge labeled by $\tbox{w}$ from $C \in V_{\square}$ to $X \in V_{\roundss}$ if $(\tbox{w}.\hat{X}) \in C$.
\end{enumerate}

\begin{figure}
    \centering
    
    \begin{tikzpicture}[node distance=1.5cm]
    %\node[circle, itria] {};
    
    
    
    
    \node (g1) [ yshift=-5cm, draw=black, shape=circle]{X};
    \node (g2) [above right of=g1, xshift=0.7cm, draw=black, shape=rectangle]{$C_1$};
    \node (g3) [below  right of=g1,xshift=0.7cm, , draw=black, shape=rectangle]{$C_2$};
    \node (g4) [above right of=g2, xshift=0.7cm,, draw=black, shape=circle]{Y};
    \node (g5) [below right of=g2,xshift=0.7cm,, draw=black, shape=circle]{Z};
    
    \path[draw=black, ->] (g1) -> node [above]{}(g2) ;
    \path[draw=black, ->] (g1) -> node [above]{}(g3) ;
    \path[draw=black, ->] (g2) -> node [above]{\small{box($\alpha$)}}(g4) ;
    \path[draw=black, ->] (g2) -> node [above]{\small{box($\beta$)}}(g5) ;
    
    
    
    \end{tikzpicture}
    \caption{Bipartite graph B}
\end{figure}  


\subsection{Winning Condition via Parity Game}

For now, we only constructed a bipartite graph from the formulas without taking the winning condition given by the B\"uchi automaton $A$ into consideration.
To this end, we want to use a cross product construction of $B$ and $A$.

This is problematic, since $A$ may be non-deterministic.
If we let the players resolve the non-determinism of the automaton in any way (i.e. by just taking the cross product of $A$ and $B$), this will change the semantics of the game in an unwanted way.
We elaborate on this in Section~\ref{sec:cheating}.

To avoid this problem, we need to determinize $A$, but deterministic Büchi automata are strictly weaker than NBAs, 
Therefore, we convert the NBA A to a parity automaton $parity(A)$ and determinize it to obtain a deterministic Parity automaton $det(parity(A))$ that is exponential in the size of $A$.

The cross product of $det(parity(A))$ and $B$ will yield a parity game on a finite graph.
Solving the context-free $\omega$-inclusion game then amounts to solving this parity game.

Due to positional determinacy of parity games, we know that from every position of the cross-product automaton either refuter or prover has a positional winning strategy. %In particular, this holds for the starting node of $A'_{game}$. Thus we have the following two cases: Either refuter wins from starting position $n_0$ by following his (winning) strategy of refuter wins from $n_0$ and thus the moves (and thus strategy) chosen by refuter do not matter. Therefore, the strategy $$c: M_A \times N \rightarrow 2^{M_A \times N} $$ of refuter can be fixed before the actual game and does no need to be adapted to the moves of refuter.
This means that we can fix an appropriate strategy for refuter in form of an extended choice function
\[
c: M_A \times N \rightarrow 2^{M_A \times N}
\]
before the actual game without changing the outcome of the game. This means that if refuter can win the game, we can fix this strategy c beforehand and it does not need to be adapted to the moves of prover during the play for refuter to win. If however refuter cannot win the game, the fixation of a strategy for prover will not change the outcome.\\
We will use this knowledge later to construct an alternative algorithm to decide which wins the game by iterating over all the possible extended choice functions and using this fixed strategy to decide the winner.


\subsection{Algorithm}
The following algorithm can decide which player wins:

\begin{enumerate}
    \item
    Construct and solve the extended system of equations as defined above.
    \item
    Construct bipartite graph $B$ from the solution of the system of equations as described above.
    \item
    Construct the cross-product automaton of $B$ and the determinized version of the parity automaton constructed from NBA $A$.
    \item
    Solve the parity game $B \times det(parity(A))$.
    The solution to the original problem is obtained by checking whether refuter wins the parity game from $(S, q_{0,det(parity(A))})$.
\end{enumerate}


\subsection{Complexity}
The steps of the algorithm above have the following complexity:
\begin{enumerate}
    \item  $\Rightarrow$ $\mathsf{2EXPTIME}$
    
    \item The bipartite graph B has the following size:\\
    It has vertex set $V=V_{\square} \dotcup V_{\roundss} \subseteq N \dotcup \mathcal{P}(N \times M_A)$  of size $|N|+2^{|N|\cdot 2^|Q|}$.\\
    The transitions are of the following form:
    $$ X \xrightarrow{\epsilon} C \subseteq \mathcal{P}(N \times M_A) \text{, if C is the image of a choice function on sol(X)}$$ 
    $$C \xrightarrow{box(\alpha)} Y \text{, if (Y,box($\alpha$))} \in C $$
    and thus there exist at most $|N|\cdot2^{|N|\cdot 2^{|Q|}} + \underbrace{2^{|N|\cdot2^{|Q|}}}_\text{number of Cs}\cdot\underbrace{|N|2^{|Q|}}_\text{size of Cs}\cdot\underbrace{3^{|Q|^2}}_\text{coding word} $ transitions.\\
    $\Rightarrow $ $\mathsf{2EXP}$
    
    \item  Determining the winner of a parity game is in $NP \cap co-NP$, on an input of size 2EXP (B has size $\mathsf{2EXP}$, det(parity(A)) size $\mathsf{EXP}$). Thus we need $2EXP \cap co-2NEXP \geq 2EXP$ time to solve this problem.  
\end{enumerate}


==> content/prelims.tex <==
\section{Preliminaries boxes}

\subsection{Basics}
\rfm{Language of a sentential form needed in Section 3 (elsewhere?)}
    where $\lang{a} = a$ for terminals $a$, $\lang{X} = \lang{G_X}$ (where $G_X$ is the grammar $G$ with $X$ as initial symbol), and $\lang{\alpha \beta} = \lang{\alpha} . \lang{\beta}$.

\rfm{We should say this once and for all.}
\footnote{We use the term $\omega$-language to mean a language of infinite words.}

\subsection{Transition boxes for \Buechi automata}

We want to characterize how a non-deterministic finite automaton can behave when processing a word. We use transition boxes to capture the possible state changes of an automaton induced by a word.

\begin{definition}
\label{def:boxes_nfa}
    Given a NFA $A$, whose set of states is $Q$, a \emph{transition box} for $A$ is an element of
    \[
        \Boxes_{NFA}(A) =
        \pwrset{  Q \times Q }
        .
    \]
\end{definition}

To get a better understanding of the relation between boxes and equivalence classes, we define the following equivalence relation.

\begin{definition}
\label{def:boxes_equivrel_nfa}
    Let $A$ be a NFA over $\Sigma$ and let $v, w \in \Sigma^*$.
    
    We define the equivalence relation on $\Sigma^*$ induced by the behavior of $A$ by
    \[
        w \sim^{NFA}_A v
        \hspace*{0.5cm} iff \hspace*{0.5cm}
        \forall q, q' \in Q: q \overset{w}{\to} q' \iff q \overset{w}{\to} q'
        .
    \]
\end{definition}
    
\begin{remark}
\label{rem:boxes_composition_nfa}
    Each box $\tboxr \in \Boxes_{NFA}(A)$ defines a set of words by
    \begin{center}
        \begin{tabular}{rcrll}
            $w \in \lang{\tboxr}$ 
            & iff
            &
            & $\forall (q, q') \in \tboxr:$
            & $q \overset{w}{\to} q'$\\
            & & and
            & $\forall (q, q') \not\in \tboxr:$
            & $q \not\overset{w}{\to} q'$
            .\\
        \end{tabular}
    \end{center}
    
    Whenever $L(\tboxr)$ is non-empty, is is actually an equivalence class of $\sim^{NFA}_A$, and every equivalence class of $\sim^{NFA}_A$ occurs as $L(\tboxr)$ for some box.
    
    Note that there is a map $\tbox{-}$ which maps each word $w$ to the box $\tbox{w}$ such that $w \in L(\tbox{word})$.
    For single letters $a$, we can construct $\tbox{a}$ directly from the transition relation of the automaton:
    \[
        \tbox{a}
        = \Set{ (q,q') }{ q \overset{a}{\to} q' \text{ in } A }
        .
    \]
    We associate the identity box $\id$ to the the empty word:
    \[
        id = \tbox{\epsilon}
        = \Set{ (q,q)}{ q \in Q}
        .
    \]
    Given two boxes $\tboxr, \tboxt$, we may compose them to get the box
    \[
        \tboxr;\tboxt = \Set{ (q,q'')}{ \text{ there are } (q,q') \in \tboxr, (q',q'') \in \tboxt}
        .
    \]
\end{remark}

\begin{remark}
\label{rem:box_composition_assoc}
    \begin{enumerate}[a)]
        \item
            Box composition is associative.
        \item
            The identity box $\id$ is the (left- \& right-)neutral element with respect to box composition.
        \item
            The set of boxes with box composition is a monoid.
        \item
            The map
            $\tbox{-} : \Sigma^* \to \Boxes_{NFA}(A)$
            which maps each word $w$ to the unique box $\tbox{w}$ such that $w \in \lang{\tbox{w}}$ is a homomorphism of monoids.
            
            In particular: if $w \in \lang{\tboxr}, v \in \lang{\tboxt}$, then $w.v \in \lang{\tboxr;\tboxt}$.
        \item
            The image of this map are exactly the boxes $\tboxr$ with $L(\tboxr) \neq \emptyset$.
            Those boxes can be obtained by iteratively composing boxes until no new boxes are created anymore, starting with the identity box and the boxes corresponding to single letters.
    \end{enumerate}
\end{remark}
 
\begin{remark}
\label{rem:box_count}
    There are up to $2^{|Q|^2}$ many boxes.
    
    Note that there are only $2^{|Q|}$ subsets of states and therefore only
    $\left( 2^{|Q|} \right)^2$ many pairs of states, i.e. constructing all boxes can be more expensive than constructing the powerset-automaton.
\end{remark}
 
\begin{example}
\label{ex:boxes_simple}
    The following figure shows all relevant boxes for the automaton from Example \ref{ex:automaton_simple}. The four dashes on each side of a box indicate the control states $q_0, ..., q_3$.
    
    \centering
    \subimport{tikz/}{boxes_simple}
\end{example}



When dealing with \Buechi automata, we need to keep track whether we have seen a final state while doing a sequence of transition. We will do this by adding a flag to each transition.

\begin{definition}
    \label{def:boxes_nba}
    Given a NBA $A$, whose set of states is $Q$, a transition box for $A$ is an element of
    \[
        \Boxes'_{NBA}(A)
        =
        \Set
        { \tboxr \in  \pwrset{  Q \times Q \times \B }   }
        { \forall q, q' \in Q: \ (q,q',1), (q,q',0) \text{ not both in } \tboxr}
        .
    \]
\end{definition}

\begin{remark}
\label{rem:boxes_equivrel_nba}
    The same theory as above carries over to NBAs:
    
    We may define the equivalence relations $\sim^f_A$ and $\sim^{NBA}_A$ on finite words by
    
    \begin{center}
        \begin{tabular}{lllrl}
            &$w \sim^{f}_A v$ & $iff$ & $ \forall q, q' \in Q:$ &  \\
             &&&  & $q \overset{w}{\to} q'$ with at least one intermediary final state\\
             &&& $iff$  & $q \overset{w}{\to} q'$ with at least one intermediary final state \\
            and &&&&\\ 
            & $w \sim^{NBA}_A v$ & $iff$ &
            \multicolumn{2}{l}{$w \sim^{NFA}_A v \ \text{ and } \ w \sim^f_A v$}
        \end{tabular}
    \end{center}

    
    Each box $\tboxr \in \Boxes^{NBA}(A)$ defines the set of words $w$ such that
    \begin{itemize}
        \item
        $A$ can go from $q$ to $q'$ while processing $w$ if and only if\\either $(q,q',0)\in \tboxr$ or $(q,q',1) \in \tboxr$
        \item
        $A$ can go from $q$ to $q'$ and sees a final state during these transitions while processing $w$ if and only if $(q,q',1) \in \tboxr$
    \end{itemize}
    
    Each single letter of the input alphabet can be associated to the box
    
    \begin{center}
        \begin{tabular}{llll}
            $\tbox{a}$ & $ = $ & & $\Set{ (q,q',1) }{ q \overset{a}{\rightarrow} q' \text{ in } A \text{ and } q \text{ or } q' \in Q_F}$\\
            & & $\cup$ & $\Set{ (q,q',0) }{ q \overset{a}{\rightarrow} q' \text{ in } A \text{ and neither } q \text{ nor } q' \in Q_F}$\\
        \end{tabular}
    \end{center}
    
    Given two boxes $\tboxr, \tboxt \in \Boxes$, we can define their \emph{composition} $\tboxr;\tboxt$ by
    
    \begin{center}
        \begin{tabular}{lllll}
            $\tboxr;\tboxt$ & $ = $ & & $\{ (q,q'',1) \ |$ &
            $ \exists q': (q,q',x) \in \tboxr,
            \ (q',q'',y) \in \tboxt,
            \ \max(x,y) = 1 \}$\\
            & & $\cup$ & $\{ (q,q'',0)\ |$ &
            $ \exists q^*: (q,q^*,0) \in \tboxr,
            \ (q^*,q'',0) \in \tboxt,
            $\\
            & & & & $\nexists q':  (q,q',x) \in \tboxr,
            \ (q',q'',y) \in \tboxt,
            \ \max(x,y) = 1 \}$
        \end{tabular}
    \end{center}
    
    Just as above, non-empty equivalence classes of $\sim^{NBA}_A$ are in one-to-one correspondence to boxes with non-empty sets of words, and all such boxes can be constructed by composing boxes starting from the boxes for single letters.
    
    Note that the identity box for this type of boxes is 
    \[
        \Set{ (q,q,0) }{ q \in Q}
        .
    \]
\end{remark}

\begin{remark}
    Later, it will be helpful to differentiate between the empty word $\epsilon$ and other words $w$ with $\tbox{w} = \Set{ (q,q,0) }{ q \in Q}$. To do this, we introduce a special identity box $\fid$.
    
    It acts as neutral element with respect to box composition:
    \[
        \fid;\tboxr = \tboxr;\fid = \tboxr
        .
    \]
    Note that with this additional box, the $\Set{ (q,q,0) }{ q \in Q}$ is not neutral anymore since
    \[
        \fid; \Set{ (q,q,0) }{ q \in Q} = \Set{ (q,q,0) }{ q \in Q}
        .
    \]
\end{remark}

\begin{definition}
    \label{def:boxes_nba_with_fake}
    Given a NBA $A$, the set of transition box for $A$ is
    \[
        \Boxes_{NBA}(A) 
        =
        \Boxes'_{NBA}(A)
        \dotcup
        \set{ \fid }
        .
    \]
    It is a monoid with respect to box composition and $\fid$ as identity. The map $\tbox{-} : \Sigma^* \to \Boxes_{NBA}(A)$ is a monoid homomorphism with $\tbox{\epsilon} = \fid$.
    
    Note that each NFA-box can be obtained by projecting each triple in the corresponding NBA-box to the first two components (where we project $\id$ to $\tbox{\epsilon}$).

    Furthermore, in the rest of this article, the context clearly indicates which automaton is used, so we will not reflect this dependency in the notation. Altogether, we will just write $\Boxes$ instead of $\Boxes^{NBA}(A)$.
\end{definition}

\begin{lemma}
    \begin{enumerate}[a)]
        \item
            Given $q,q'$ control states of $A$, the language
            \[
                \lang_{q,q'}
                =
                \Set{ w \in \Sigma^* }
                { q \stackrel{w}{\to} q'}  
            \]
            is regular.
        \item
            Given $q,q'$ control states of $A$, the language
            \[
                \lang_{q,q'}^f
                =
                \Set{ w \in \Sigma^* }
                { q \stackrel{w}{\to} q' \text{ with an intermediary final state}}  
            \]
            is regular.
        \item
            Given a box $\tboxr \in \Boxes$, its equivalence class of words $\lang{\tboxr}$ is regular.   
    \end{enumerate}
    \begin{proof}
        \begin{enumerate}[a)]
            \item
                We can construct an NFA deciding $\lang_{q,q'}$ by changing the initial state of $A$ to $q$ and making $q'$ the unique final state.
            \item
                Similar to a). Create two copies of $A$. The initial state is the $q$ in the first copy, the unique final state is $q'$ in the second copy. Change from the first to the second copy as soon as we have seen a final state of $A$ (and treat the case where $q$ or $q'$ is final correctly).
            \item
                \[
                    \lang{\fid} = \set{ \epsilon }
                \]
                For any other box, we have
                \[
                    \lang{\tboxr}
                    =
                    \bigcap
                        \limits_{
                            \substack{ q,q' s.t. \\ (q,q',1) \in \tboxr }
                        }
                        \lang_{q,q'}^f
                    \cap
                    \bigcap
                        \limits_{
                            \substack{ q,q' s.t.\\  (q,q',0) \in \tboxr }
                        }
                        \left(
                            \lang_{q,q'} \cap \overline{ L_{q,q'}^f }
                        \right)
                    \cap
                    \bigcap
                        \limits_{
                            \substack{ q,q' s.t. \\ (q,q',1) \not\in \tboxr, \\ (q,q',0) \not\in \tboxr}
                        }
                        \overline{ \lang_{q,q'} }
                    \cap
                        \left(
                            \Sigma^* \setminus \set{ \epsilon }
                        \right)
                \]
                which is a finite intersection of regular languages.
        \end{enumerate}
    \end{proof}
\end{lemma}

\begin{example}
\label{ex:boxes_ab}
    The following figure shows all relevant NBA-boxes for the automaton from Example \ref{ex:automaton_ab}. The dot on an arrow indicates that we have seen a final state by doing this transition. 
    
    \centering
    \subimport{tikz/}{boxes_ab}
\end{example}

\begin{example}
\label{ex:boxes_reqack}
    The following figure shows some relevant boxes for the automaton from Example \ref{ex:automaton_reqack}.
    
    \centering
    \subimport{tikz/}{boxes_reqack}
\end{example}


\begin{remark}
    A transition box $\tboxr \in \Boxes$
    defines a labeled directed graph:
    \begin{itemize}
        \item
            every state represents a vertex ,
        \item
            there is an arc from $q$ to $q'$ if and only if $(q,q',x) \in \tboxr$ for some $x \in \set{0, 1}$,
        \item
            and this arc is labeled by $1$ if $x = 1$ and $0$ otherwise.
    \end{itemize}
    
   
\end{remark}

\begin{example}
\label{ex:box_as_graph}

    The box $\tbox{req}$ from Example \ref{ex:boxes_reqack} as labeled graph.
    
    \centering
    \subimport{tikz/}{box_as_graph}
\end{example}

\begin{remark}
    In the rest of this article, we will identify the following each objects with each other:
    \begin{enumerate}[a)]
        \item
            Transition boxes $\tboxr \in \Boxes$.
        \item
            The equivalence class of words defined by $\tboxr$, i.e. the regular language $\lang{\tboxr}$.
        \item
            The labeled directed graph defined by $\tboxr$.
    \end{enumerate}
\end{remark}


As a running example, we consider $G = (\set{ X, Y }, T, P, X)$ with terminal alphabet $T=\set{ req, ack, s, t }$ and  productions $P=\set{X \rightarrow req \ Y \ ack, X\rightarrow  XX, Y \ \rightarrow s \ Y \ t, Y\rightarrow \varepsilon}$. 
The grammar generates the language
    \[
        \lang{G} 
        =
        \Set{ \big(req (s^{n_i}  t^{n_i})  ack \big)^m }{ m \geq 1, n_i \geq 0 \ \forall i \in \oneto{m}}
        .\vspace{0.1cm}
    \]
\begin{minipage}{7cm}
The automaton $A$ over the same alphabet $T$ is depicted to the right. 
Its language is the set of words $w$ such that every request is followed by an acknowledge:
\end{minipage}\hspace{0.4cm}
\begin{minipage}{5cm}
\scalebox{0.8} { \subimport{tikz/}{automaton_reqack}}
\end{minipage}
    \begin{center}
        \begin{tabular}{rll}
            $\lang{A}$
            &$= (T^* \ req \ T^* \ ack \ T^*)^*$
            &$= \Set{ w \in T^*}
            { \forall i \in \zeroto{|w|-1}: w_i = req \Rightarrow \exists j > i: w_j = ack}$,\\
            $\olang{A_3}$
            &$= (T^* \ req \ T^* \ ack \ T^*)^\omega$
            &$=
            \Set{ w \in \Sigma^\omega}
            { \forall i \in \N: w_i = req \Rightarrow \exists j > i: w_j = ack}$
            .
        \end{tabular}
    \end{center}
  
    This implies the condition that if a word contains infinitely many requests, it has to contain infinitely many acknowledges. The automaton does not check that every request has a corresponding acknowledge, since this condition is not $\omega$-regular.


==> style/algo.tex <==
% ############
% ALGORITHMS
% ############

% algorithms
\usepackage{algorithmicx}
\usepackage{algpseudocode}

% code for "indentation guide"-style verticle lines
\makeatletter
\def\therule{\makebox[\algorithmicindent][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%

\newtoks\therules% Contains rules
\therules={}% Start with empty token list
\def\appendto#1#2{\expandafter#1\expandafter{\the#1#2}}% Append to token list
\def\gobblefirst#1{% Remove (first) from token list
  #1\expandafter\expandafter\expandafter{\expandafter\@gobble\the#1}}%

\let\oldState\State
\def\LState{\oldState\unskip\the\therules}% New line-state
\let\State\LState
\let\Cmd\LState

\def\pushindent{\appendto\therules\therule}%
\def\popindent{\gobblefirst\therules}%
\def\printindent{\unskip\the\therules}%
\def\printandpush{\printindent\pushindent}%
\def\popandprint{\popindent\printindent}%

\algdef{SE}[WHILE]{While}{EndWhile}[1]
  {\printandpush\algorithmicwhile\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicwhile}%
\algdef{SE}[FOR]{For}{EndFor}[1]
  {\printandpush\algorithmicfor\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicfor}%
\algdef{S}[FOR]{ForAll}[1]
  {\printindent\algorithmicforall\ #1\ \algorithmicdo}%
\algdef{SE}[LOOP]{Loop}{EndLoop}
  {\printandpush\algorithmicloop}
  {\popandprint\algorithmicend\ \algorithmicloop}%
\algdef{SE}[REPEAT]{Repeat}{Until}
  {\printandpush\algorithmicrepeat}[1]
  {\popandprint\algorithmicuntil\ #1}%
\algdef{SE}[IF]{If}{EndIf}[1]
  {\printandpush\algorithmicif\ #1\ \algorithmicthen}
  {\popandprint\algorithmicend\ \algorithmicif}%
\algdef{C}[IF]{IF}{ElsIf}[1]
  {\popandprint\pushindent\algorithmicelse\ \algorithmicif\ #1\ \algorithmicthen}%
\algdef{Ce}[ELSE]{IF}{Else}{EndIf}
  {\popandprint\pushindent\algorithmicelse}%
\algdef{SE}[PROCEDURE]{Procedure}{EndProcedure}[2]
   {\printandpush\algorithmicprocedure\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicprocedure}%
\algdef{SE}[FUNCTION]{Function}{EndFunction}[2]
   {\printandpush\algorithmicfunction\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicfunction}%
\makeatother

% C-style comments
\renewcommand {\algorithmiccomment}[1]
    {\hfill $/ \!/$ #1}
   
% return on new line
\let\oldReturn\Return
\renewcommand{\Return}{\LState\oldReturn}

% commands like in algorith2e
\newcommand {\ForLoop} [2]
{
    \For {#1}
        #2
    \EndFor
}

\newcommand {\WhileLoop} [2]
{
    \While {#1}
        #2
    \EndWhile
}

\newcommand {\IfCond} [2]
{
    \If {#1}
        #2
    \EndIf
}

\newcommand {\IfElseCond} [3]
{
    \If {#1}
        #2
    \Else
        #3
    \EndIf
}

% environments
\newenvironment {forenv} [1]
{
    \For { #1 }
}
{ 
    \EndFor
}

    
\newenvironment {whileenv} [1]
{
    \While { #1 }
}
{ 
    \EndWhile
}

\newenvironment {ifenv} [1]
{
    \If { #1 }
}
{ 
    \EndIf
}


==> style/commands.tex <==
% ##########
% COMMANDS
% ##########

% custom emph
\newcommand {\emphbf}[1]
{ \emph{#1} }

% bold + italic
\newcommand {\textbfit} [1]
{ \textbf{\textit{#1}} }

% monospace (+ bold & italic)
\newcommand {\mono} [1]
{ \texttt {#1} }

\newcommand {\monobf} [1]
{ \texttt {\bfseries #1} }

\newcommand {\monobfit} [1]
{ \texttt {\bfseries \itshape #1} }

\newcommand {\monoit} [1]
{ \texttt {\itshape #1} }

% fake capital greek letters
\newcommand {\Alpha} {A}
\newcommand {\Beta} {B}
\newcommand {\Epsilon} {E}
\newcommand {\Zeta} {Z}
\newcommand {\Eta} {H}
\newcommand {\Iota} {I}
\newcommand {\Kappa} {K}
\newcommand {\Mu} {M}
\newcommand {\Tau} {T}
\newcommand {\Chi} {X}

\providecommand\B{}
\renewcommand {\B} {{\mathbb B}}
\newcommand {\N} {{\mathbb N}}
\newcommand {\A} {{\mathbb A}}
\newcommand {\Z} {{\mathbb Z}}
\newcommand {\R} {{\mathbb R}}
\providecommand{\C}{}
\renewcommand {\C} {{\mathbb C}}
\newcommand {\Q} {{\mathbb Q}}
\newcommand {\D} {{\mathbb D}}
\newcommand {\F} {{\mathbb F}}
\newcommand {\E} {{\mathbb E}}
\providecommand {\G} {}
\renewcommand {\G} {{\mathbb G}}
\newcommand {\K} {{\mathbb K}}
\newcommand {\V} {{\mathbb V}}
\renewcommand {\P} {{\mathbb P}}
\renewcommand {\H} {{\mathbb H}}

% caligraphic letters
\newcommand {\calA} {\mathcal{A}}
\newcommand {\calB} {\mathcal{B}}
\newcommand {\calC} {\mathcal{C}}
\newcommand {\calD} {\mathcal{D}}
\newcommand {\calE} {\mathcal{E}}
\newcommand {\calF} {\mathcal{F}}
\newcommand {\calG} {\mathcal{G}}
\newcommand {\calH} {\mathcal{H}}
\newcommand {\calI} {\mathcal{I}}
\newcommand {\calJ} {\mathcal{J}}
\newcommand {\calK} {\mathcal{K}}
\newcommand {\calL} {\mathcal{L}}
\newcommand {\calM} {\mathcal{M}}
\newcommand {\calN} {\mathcal{N}}
\newcommand {\calO} {\mathcal{O}}
\newcommand {\calP} {\mathcal{P}}
\newcommand {\calQ} {\mathcal{Q}}
\newcommand {\calR} {\mathcal{R}}
\newcommand {\calS} {\mathcal{S}}
\newcommand {\calT} {\mathcal{T}}
\newcommand {\calU} {\mathcal{U}}
\newcommand {\calV} {\mathcal{V}}
\newcommand {\calW} {\mathcal{W}}
\newcommand {\calX} {\mathcal{X}}
\newcommand {\calY} {\mathcal{Y}}
\newcommand {\calZ} {\mathcal{Z}}


==> style/definitions.tex <==
% ##################
% DEFINITIONS
% ##################

%
% Basic stuff
%

\newcommand { \from }
{ \leftarrow }

\newcommand {\Rplus} 
{ \R_{>0} }

\newcommand {\true}
{\mono{true}}

\newcommand {\false}
{\mono{false}}

\newcommand { \ifalse }
{ \mathit{false} }

\newcommand { \itrue }
{ \mathit{true} }

\newcommand {\oneto} [1]
{\left\{ 1, \ldots, #1\right\}}

\newcommand {\zeroto} [1]
{\left\{ 0, \ldots, #1\right\}}

\newcommand {\arity} [1]
{ {\scriptstyle / #1 } }

% matrix dimensions
\newcommand {\sz} [2]
{ #1 \raisebox{0.5pt} {\text{\;\!\tiny x\;\!}} #2}

\newcommand {\nsz} [2]
{ #1 \raisebox{0.5pt} {\text{\;\!\small x\;\!}} #2}

% small @
\newcommand {\at}
{
    \raisebox{0.5mm}{\scalebox{0.7}[0.7]{@}}
}

% corresponds to
\newcommand\corrto{%
    \let\savearraystretch\arraystretch
    \renewcommand\arraystretch{0.3}
    \begin{array}{c}
        \stretchto{
            \scalerel*[\widthof{=}]{\wedge}
            {\rule{1ex}{3ex}}%
        }{0.5ex}\\ 
        =%
    \end{array}
    \let\arraystretch\savearraystretch
}

% stacked logical operators
\newcommand{\wedgevee}
{
    \mathrel{\substack{\wedge\\\vee}}
}
\newcommand{\veewedge}
{
    \mathrel{\substack{\vee\\\wedge}}
}

%
% Sets
%

\newcommand {\set} [1]
{ \left\{ #1 \right\} }

\newcommand {\Set} [2]
{ \left\{ #1 \ \middle| \ #2 \right\} }

\newcommand {\smallset} [2]
{ \{ #1 \mid #2 \} }

\newcommand {\ideal} [1]
{ \langle \ #1 \ \rangle}

\newcommand {\Ideal} [2]
{ \langle \ #1 \mid #2 \ \rangle}

\newcommand {\pwrset} [1]
{ {\mathcal P} \left( #1 \right)}

%
% Set operations
%

\newcommand* {\medcap}
{ \mathbin{\scalebox{1.5}{\ensuremath{\cup}}} }
\newcommand* {\medcup}
{ \mathop{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}} } 
\newcommand* {\hugecup}
{ \mathop{\mathbin{\scalebox{3}{\ensuremath{\cup}}}} }

\newcommand {\bigdotcup}
{\ensuremath{\mathop{\mathaccent\cdot{\bigcup}}}}
\newcommand {\dotcup}
{\ensuremath{\mathop{\mathaccent\cdot\cup}}}

% disjoint union
\makeatletter
\providecommand*{\bigcupdot}{%
    \mathbin{%
        \mathpalette\@bigcupdot{}%
    }%
}
\newcommand*{\@bigcupdot}[2]{%
    \ooalign{%
        $\m@th#1\bigcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

\makeatletter
\providecommand*{\cupdot}{%
    \mathbin{%
        \mathpalette\@cupdot{}%
    }%
}
\newcommand*{\@cupdot}[2]{%
    \ooalign{%
        $\m@th#1\cup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

%
% Logic
%
\newcommand {\Fzero} {\calF_0}
\newcommand {\dedFzero} {\vdash_{\calF_0}}
\DeclareDocumentCommand \FO { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO} }
    { \text{FO} \left( #1 \right) }
}
\newcommand {\dedG} {\vdash_{G}}
\newcommand {\dedRes} {\vdash_{\mathit{Res}}}
\newcommand {\sem}[1]
{	\left\llbracket #1 \right\rrbracket }
\newcommand {\Sko} {\mathsf{Sko}}
\DeclareDocumentCommand \FOneq { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO}^{\neq} }
    { \text{FO}^{\neq} \left( #1 \right) }
}
\DeclareDocumentCommand \FOcl { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO}_{\mathit{abg}} }
    { \text{FO}_{\mathit{abg}} \left( #1 \right) }
}
\newcommand {\Dherbrand} {D_{\calH}}

% inverse models
\makeatletter
\providecommand*{\Dashv}{%
    \mathrel{%
        \mathpalette\@Dashv\vDash
    }%
}
\newcommand*{\@Dashv}[2]{%
    \reflectbox{$\m@th#1#2$}%
}
\makeatother

% logical equivalence (\models \ismod)
\newcommand{\lequiv}{\vDash\hspace{-2pt}\Dashv}

% cons / folg
\DeclareMathOperator {\Folg} {Folg}
\DeclareMathOperator {\Cons} {Cons}


%
% Complexity
%

\newcommand {\bigO} [1]
{ \calO \left( {#1} \right) }

\newcommand {\smallO} [1]
{ o \left( #1 \right) }

\newcommand {\bigOmega} [1]
{ \Omega \left( #1 \right) }

\newcommand {\smallOmega} [1]
{ \omega \left( #1 \right) }

\newcommand {\bigTheta} [1]
{ \Theta \left( #1 \right) }

% blank symbol
%\newsavebox{\textvisiblespacebox}
%\savebox{\textvisiblespacebox}{\texttt{a}}
%\newcommand\vartextvisiblespace[1][\wd\textvisiblespacebox]{%
%    \makebox[#1]{\kern.1em\rule{.4pt}{.3ex}%
%        \hrulefill%
%        \rule{.4pt}{.3ex}\kern.1em}%
%}
%\newcommand{\blank}{\vartextvisiblespace}% For ease-of-use
\newcommand{\blank}{\texttt{\char32}}% For ease-of-use

\newcommand {\LOGSPACE}
{\mono{L}}
\newcommand {\NLOGSPACE}
{\mono{NL}}
\newcommand {\PTIME}
{\mono{P}}
\newcommand {\NPTIME}
{\mono{NP}}
\newcommand {\PSPACE}
{\mono{PSPACE}}
\newcommand {\EXPTIME}
{\mono{EXP}}
\newcommand {\EXPSPACE}
{\mono{EXPSPACE}}

%
% Graphs
%

\newcommand {\paths} [2]
{ { \calP \left( {#1}, {#2} \right)} }

\newcommand {\cycles} [1]
{ \calC \left( #1 \right)}

\newcommand {\cyclesne} [1]
{ \calC^{\neq \epsilon} \left( #1 \right)}


%
% Automata theory
%

\newcommand {\tow} [1]
{ \overset{#1}{\to} }


\DeclareDocumentCommand \lang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL }
    { \calL \left( #1 \right) }
}
\newcommand {\langm}
{ \calM }
\DeclareDocumentCommand \olang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL^\omega }
    { \calL^\omega \!\left( #1 \right) }
}

\DeclareMathOperator {\Monoid} {M}
\DeclareMathOperator {\Boxes} {B}

% 
% Algebraic geometry, Computer algebra
% 

\providecommand{\x}{}
\renewcommand {\x} {\underline{x}}
\newcommand {\xs} {\underline{xs}}
\newcommand {\p} {\underline{p}}

\newcommand {\polyr} { K [ \x ] }

\newcommand {\polyrQ} { \Q [ \x ] }
\newcommand {\polyrC} { \C [ \x ] }

\newcommand {\polyrs} { K [ \xs ] }
\newcommand {\polyrwo} [1]
{ K [ x_j \ | \ j \neq #1 \ ] }
\newcommand {\polyrwoi} { K [ x_j \ | \ j \neq i \ ] }
\newcommand {\polyrQwoi} { \Q [ x_j \ | \ j \neq i \ ] }
\newcommand {\polyrQwo} [1]
{ \Q [ x_j \ | \ j \neq #1 \ ] }

\newcommand {\laurentr} { K [ \x^{\pm 1} ] }
\newcommand {\laurentrQ} { \Q [ \x^{\pm 1} ] }

\newcommand {\Qxs} { \Q [ \xs ] }

\newcommand {\tropring} {(\R \cup \{ -\infty\})}

\newcommand {\aff} [2] {\A ^{#1} _{#2}}
\newcommand {\affn} [1] {\A ^{n} _{#1}}
\newcommand {\affnk} {\A ^{n} _{K}}

\newcommand {\projs} [2] {\P ^{#1} _{#2}}
\newcommand {\projn} [1] {\P ^{n} _{#1}}
\newcommand {\projnK} {\P ^{n} _{K}}

\newcommand {\tor} [2]
{T ^{#1} _{#2}}
\newcommand {\torn} [1]
{T ^{n} _{#1}}
\newcommand {\tornK} {T ^{n} _{K}}

\newcommand {\puis} [1]
{#1\{ \! \{t\} \! \}}
\newcommand {\puisK} {K\{ \! \{t\} \! \}}
\newcommand {\puisC} {\C\{  \! \{t\} \! \}}

\DeclareMathOperator {\LT} {LT}
\DeclareMathOperator {\LC} {LC}
\DeclareMathOperator {\LM} {LM}

\DeclareMathOperator {\InitOp} {in}
\newcommand {\Init} [2]
{ \InitOp_{#1} \left( #2 \right)}

\DeclareMathOperator {\troppoly} {troppoly}

\DeclareMathOperator {\TropOp} {Trop}
\newcommand {\Trop} [1]
{ \TropOp \left( #1 \right)}

%
% Polyhedrons
%

\DeclareMathOperator {\cone} {cone}

\DeclareMathOperator {\IntOp} {Int}
\newcommand {\Int} [1]
{ \IntOp \left( #1 \right)}

\DeclareMathOperator {\RelIntOp} {relInt}
\newcommand {\RelInt} [1]
{ \RelIntOp \left( #1 \right)}

\DeclareMathOperator {\Suppop} {Supp}
\newcommand {\Supp} [1]
{\Suppop \left( #1 \right)}

%
% Master thesis specific
%

\newcommand {\subsets} [2]
{ \Lambda\left(#1, #2\right) }

\DeclareMathOperator {\BoundeOp} {Bound^e}
\newcommand {\Bounde} [2]
{ \BoundeOp_{#1} \left( #2 \right) }
\newcommand {\Boundei} [1]
{ \Bounde{i} {#1}}
\newcommand {\Boundes} [1]
{ \Bounde{1} {#1}}

\DeclareMathOperator {\BoundpOp} {Bound^p}
\newcommand {\Boundp} [2]
{ \BoundpOp_{#1} \left( #2 \right) }
\newcommand {\Boundpi} [1]
{ \Boundp{i} {#1}}
\newcommand {\Boundps} [1]
{ \Boundp{1} {#1}}

%
% Abbreviations
%

\newcommand {\singular} {S\textsc{ingular} }
\newcommand {\Buechi} {{B\"uchi }}

%
% Antichains for Inclusion Games
%

% left derivation
\newcommand{\leftderive}{\Rightarrow_L}

% transition boxes
\newcommand {\tboxr}
{ \rho }
\newcommand {\tboxt}
{ \tau }
\newcommand {\tbox} [1]
{ \rho_{#1} }
\newcommand {\var} [1]
{ \Delta_{#1} }
\newcommand {\sol} [1]
{ \sigma_{#1} }

% "fake" identity
\newcommand {\fid}
{ \id }

% CNF formulas
\DeclareMathOperator {\CNF}
{ CNF }
\newcommand {\CNFE}
{ \CNF \! /_{\lsim}}

% positive formulas over boxes
\DeclareMathOperator {\BF}
{ BF }
\newcommand {\BFE}
{ \BF \! /\!_{\lsim}}

% singleton formula
\newcommand {\snglt} [1]
{ \set{ \set{ #1 } } }

% special orders
\newcommand {\lleq}
{ \Rightarrow}
%{ \models}
\newcommand {\lsim}
{ \Leftrightarrow }
%{ \lequiv }

\newcommand {\natlt}
{ \prec }
\newcommand {\natgt}
{ \succ }

\newcommand{\stateequiv} [1]
{\sim_{#1}}


% winning regions and strategies
\newcommand {\wrinclusion}
{W^{\subseteq \calL (A) }}
\newcommand {\wrnoninclusion}
{W^{\not\subseteq \calL (A) }}

\newcommand {\wstratemptiness}
{s^{= \emptyset}}
\newcommand {\wstratnonemptiness}
{s^{\neq \emptyset}}
\newcommand {\wstratinclusion}
{s^{\subseteq \lang{A} }}
\newcommand {\wstratnoninclusion}
{s^{\not\subseteq \lang{A} }}

% players
\newcommand {\round} { {\raisebox{0.1em}{{\mbox{\scaleobj{0.8}{\bigcirc}}}}} }
\newcommand {\roundss} { {\raisebox{0.1em}{{\mbox{\scaleobj{0.65}{\bigcirc}}}}} }

\newcommand {\players} { \set{\round, \square}}

\newcommand\openbigstar[1][0.7]{
    {
        \scalerel*{%
            \stackinset{c}{-.125pt}{c}{}{\scalebox{#1}{\color{white}{$\bigstar$}}}{%
                $\bigstar$}%
        }{\bigstar}
    }
}
\newcommand {\player} { {\openbigstar} }
\newcommand {\opponent} { \overline{\openbigstar} }

% other stuff
\newcommand {\ChosenBoxes} { \Set{ c(K) }{ K \in F }  }

\newcommand {\lvl}
{\mathit{lvl}} 

\DeclareDocumentCommand \level { g } % optoinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \mathit{level } }
    { \mathit{level} \! \left( #1 \right) \!  }
}

\DeclareDocumentCommand \FT { g g } % two optional arguments in curly braces
{ 
    \IfNoValueTF {#1}
    {
        {\calT}
    }
    {
        \IfNoValueTF {#2}
        {
            {\calT_{#1}}
        }
        {
            {\calT_{#1}^{#2}}   
        }
    }
}


% automata theory

\newcommand{\WMSO}{WMSO}
\DeclareMathOperator{\suc}{suc}
\newcommand{\WDSO}{WDSO}
\newcommand{\WMSONull}{\WMSO_0}

% Petri net stuff
\newcommand {\subword} {\!\preceq}


==> style/includes.tex <==
% ##########
% INCLUDES
% ##########

% images, ...
\usepackage{graphicx}

% tables (over several pages)
%\usepackage{array}
\usepackage{tabu}
%\usepackage{longtable}

% boxes in the text
\usepackage{fancybox}

% mathematic symbols
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stmaryrd} 
\usepackage{amsthm}
\usepackage{wasysym}
\usepackage{float}

% binary ops, for comparasion only
%\usepackage{shuffle} % not compatible with LIPIcs

% colored text
\usepackage{color}

% bmatrix* with alignment
\usepackage{mathtools}

% symbol scaling in math mode
\usepackage{scalerel}

% for symbol stacking
\usepackage{stackengine}

% for coloring stuff
\usepackage{xcolor}

% \include* without new page
%\usepackage{newclude}

% parse optional arguments
\usepackage{xparse}

% ????
\usepackage{bm}
\usepackage{oldgerm}
\usepackage{texdraw}
\usepackage{multirow}

% subimport
\usepackage{import}

% fix some spacing issues
\usepackage{microtype}


==> style/langEN.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: ENGLISH
% ###################################

%
% Packages
%

%\usepackage[T1]{fontenc} % WTF!?
\usepackage[english]{babel}
\usepackage{csquotes}

%
% Commands
%

\newcommand{\pts}{points}
\newcommand{\page}{Page}

\newcommand {\quot} [1] {\enquote{#1}}


==> style/misc.tex <==
% ##########
% MISC
% ##########

% FIX DELIMITERS SPACING
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

% triangle qed
\newcommand{\tqed}{\hfill \text{$\blacktriangleleft$}}

% item with arrow symbol like in Meyer's lectures
\newcommand {\itemarrow} 
{ {\raisebox{0.8mm}{\rotatebox[origin=c]{180}{$\Lsh$}}} }

% skip line (for nice enumerate / itemize)
\newcommand {\skipline}
{
    \mbox{}
    \vspace*{-0.3cm}
}

% brackets in various sizes
%\newcommand {\ob} {\big (}
%\newcommand {\obm} {\Big (}
%\newcommand {\obl} {\bigg (}
%\newcommand {\obh} {\Bigg (}
%\newcommand {\cb} {\big )}
%\newcommand {\cbm} {\Big )}
%\newcommand {\cbl} {\bigg )}
%\newcommand {\cbh} {\Bigg )}
%
%\newcommand {\osb} {\big [}
%\newcommand {\osbm} {\Big [}
%\newcommand {\osbl} {\bigg [}
%\newcommand {\osbh} {\Bigg [}
%\newcommand {\csb} {\big [}
%\newcommand {\csbm} {\Big ]}
%\newcommand {\csbl} {\bigg ]}
%\newcommand {\csbh} {\Bigg ]}



==> style/nth.tex <==
% nth.sty  version 2002/27/02 Donald Arseneau
% Ordinal numbering style, 1st 2nd 3rd 4th 5th... 12th... 101st 102nd...
%
% (Public domain: take, include, extract, whatever)
%
% In LaTeX: 
%           \usepackage[super,negative]{nth}
% where option [super] gives superscript `th'
% and option [negative] allows ``st, nd, rd'' suffixes on negative numbers.
%
% example:  \renewcommand{\thesection}{\ordinal{section}}
% or        \renewcommand{\thesection}{\@ordinal\c@section}
% or        \renewcommand{\thesection}{\nth\c@section}
%   
% In plain TeX: 
%           \input nth.sty
% use:      \nth{<number>}.
% Change formatting by redefining \nthscript and \nthtest

% modified to be also able to do things like \nth{i}
% (in this case, always "th" is used)

% ToDo:
% \nth{(n+1)} should give (n+1)^st

\usepackage{xstring}

\def\nth#1{
    \IfInteger{#1}
    {\nthH{#1}}
    {#1\nthscript{th}}
}

\def\nthH#1{% First print number:
    \expandafter\nthM \number #1\relax
    \nthscript{%
        \ifnum#1\nthtest0 th\else % negatives are all ``th'' (depending on \nthtest)
        \expandafter \nthSuff \expandafter 0\number\ifnum #1<0-\fi#1\delimiter
        \fi
    }}
    
% Minus sign using math mode:
\def\nthM#1{\if -#1\ifmmode-\else$-$\fi\else #1\fi}

% Print suffix depending on last two digits:
\def\nthSuff#1#2#3{%
    \ifx \delimiter#3% #1#2 are last two digits
    \ifnum #1=1 th%  teens are always ``th''
    \else % use appropriate suffix
    \ifcase #2 th\or st\or nd\or rd\else th\fi
    \fi
    \else % continue scanning for last two digits
    \expandafter \nthSuff \expandafter #2\expandafter #3%
    \fi}

% Formatting hook for ordinals (\let\nthscript\textsuperscript)
\def\nthscript#1{\textsuperscript{#1}}% alternate: \def\nthscript#1{$\rm^{#1}$}

% Formatting hook for all negative numbers giving ``th''
\def\nthtest{=}  % alternate: \def\nthtest{=}

%\ifx\Alph\undefined\else
%\def\ordinal#1{\expandafter\@ordinal\csname c@#1\endcsname}
%\let\@ordinal\nth
%\ProvidesPackage{smnth}[2016/05/31] % yyyy-mm-dd
%\DeclareOption{super}{\def\nthscript#1{#1}}
%\DeclareOption{negative}{\def\nthtest{<}}
%\ProcessOptions
%\fi
%    


==> style/operators.tex <==
% ##################
% OPERATORS
% ##################

\DeclareMathOperator {\characteristic} {char}
\DeclareMathOperator {\cols} {cols}
\DeclareMathOperator {\rows} {rows}
\DeclareMathOperator{\Attr}{Attr}
\DeclareMathOperator{\ann}{ann}
\DeclareMathOperator{\Ass}{Ass}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Baselocus}{Baselocus}
\DeclareMathOperator{\Bil}{Bil}
\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\Cl}{\kc\!\!\;\ell\!\:}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Cok}{Cok}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\degbound}{d}
\DeclareMathOperator{\Def}{Def}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Eig}{Eig}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\expdim}{expdim}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\GF}{GF}
\DeclareMathOperator{\ggT}{ggT}
\DeclareMathOperator{\ggt}{ggt}
\DeclareMathOperator{\Gl}{Gl}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\Graph}{Graph}
\DeclareMathOperator{\height}{height}
\DeclareMathOperator{\Hau}{Hau}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Hilb}{Hilb}
\DeclareMathOperator{\HP}{HP}
%{\HOM}[1]{\mbox{\DeclareFixedFont{\AZC}{T1}{pzc}{m}{it}{#1}\AZC Hom\,}}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\kgV}{kgV}
\DeclareMathOperator{\kgv}{kgv}
\DeclareMathOperator{\lc}{lc}
\DeclareMathOperator{\lead}{lead}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\inv}{inv}
\DeclareMathOperator{\jet}{jet}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\Mat}{Mat}
%\renewcommand{\mod}{\mbox{\rm mod }}
\DeclareMathOperator{\modality}{mod}
\DeclareMathOperator{\Mon}{Mon}
\DeclareMathOperator{\Mor}{Mor}
%\DeclareMathOperator{\mSpec}{\textswab{m}-Spec}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\NS}{NS}
\DeclareMathOperator{\Num}{Num}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\OO}{O}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Pot}{Pot}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\Preshv}{Preshv}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\Quot}{Quot}
\DeclareMathOperator{\rang}{rang}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\re}{Re}
%\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Reg}{Reg}
\DeclareMathOperator{\Sec}{Sec}
\DeclareMathOperator{\Sesq}{Sesq}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\Shv}{Shv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Sl}{Sl}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spur}{Spur}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\Syl}{Syl}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\UU}{U}
\DeclareMathOperator{\ZFK}{ZFK}
\DeclareMathOperator{\redNF}{redNF}
\DeclareMathOperator{\spoly}{spoly}
\DeclareMathOperator{\tail}{tail}
\DeclareMathOperator{\new}{new}
\DeclareMathOperator{\bin}{bin}
%\DeclareMathOperator{\st}{s.t.}


==> style/paper.tex <==
% ########################
% PAPER SPECIFIC STUFF
% ########################

% enumerate etc
\usepackage{paralist}

\theoremstyle{plain}
\newtheorem {proposition} [theorem] {Proposition}
\newtheorem {Claim} [theorem] {Claim}

\theoremstyle{definition}
\newtheorem {algo} [theorem] {Algorithm}

\sloppy
\clubpenalty = 10000 
\widowpenalty = 10000 
\displaywidowpenalty = 10000



==> style/theoremsEN.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}


==> style/tikz.tex <==
% ########################
% TIKZ
% ########################

% Includes
\usepackage{tikz}
\usepackage{pgf}

\usetikzlibrary{external}
\tikzexternalize[prefix=tikz_external/]

\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}

\tikzset{
    treenode/.style = {align=center, inner sep=0pt, text centered,
        font=\sffamily},
    arn_n/.style = {treenode, circle, white, font=\sffamily\bfseries, draw=black,
        fill=black, text width=1.5em},% arbre rouge noir, noeud noir
    arn_r/.style = {treenode, circle, red, draw=red, 
        text width=1.5em, very thick},% arbre rouge noir, noeud rouge
    arn_x/.style = {treenode, rectangle, draw=black,
        minimum width=0.5em, minimum height=0.5em},% arbre rouge noir, nil
    roundpos/.style = {treenode, circle, black, draw=black,
        minimum size=2.5em},
    squarepos/.style = {treenode, rectangle, black, draw=black,
        minimum width=2em, minimum height=2em},
}
\tikzset{
    invisible/.style={opacity=0},
    visible on/.style={alt={#1{}{invisible}}},
    alt/.code args={<#1>#2#3}{%
        \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
    },
}

\tikzset
{
    tboxoutline/.style = 
    {
        draw,
        thick,
        minimum size=6em,
        inner sep=0pt,
        outer sep=0pt,
    },
    tboxstate/.style =
    {
        minimum width=4pt,
        minimum height=2pt,
        inner sep=0pt,
        fill
    },
    tboxarrow/.style =
    {
    },
    pics/tbox/.style 2 args =
    {
        code =
        {
            \node[tboxoutline,pic actions] (-box) {};
            \foreach \i in {1,...,#1}
            {
                \path
                    (-box.north west)
                    --
                    node
                        [tboxstate,anchor=east,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-in-\i)
                        {}
                    (-box.south west);
                \path
                    (-box.north east) --
                    node
                        [tboxstate,anchor=west,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-out-\i)
                        {}
                (-box.south east);
            }
            
            \foreach \i/\j/\d in {#2}
            {
                \draw
                    [   
                        tboxarrow,
                        decoration =
                        {
                            markings,
                            mark=
                                at position 1 with
                                {
                                    \arrow[scale=1,>=triangle 45]{>}
                                }
                        }
                        ,
                        postaction={decorate}
                    ]
                    (-box-in-\i.east)
                    --
                    node
                        [pos=.5,\d]
                        {}
                    (-box-out-\j.west);
            }
        }
    },
    tbox color/.style={
        tboxstate/.append style={fill=#1},
        tboxoutline/.append style={draw=#1},
        tboxarrow/.append style={draw=#1},
    },
    trans/.style =
    {
        thick,
    },
    dot/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
        fill,
    },
    dott/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
    },
}


==> tikz/automaton_ab.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
semithick]
%\tikzstyle{every state}=[fill=red,draw=none,text=white]

\node[initial,state,accepting] (A)                    {$q_0$};
\node[state] (B) [right of=A] {$q_1$};

\path
(A) edge [bend left ] node [above]  {a} (B)
(B) edge [bend left] node [below] {b} (A);
\end{tikzpicture}

==> tikz/box_as_graph.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
semithick]
%\tikzstyle{every state}=[fill=red,draw=none,text=white]

\node[state] (A)  {$q_0$};
\node[state] (B) [right of=A] {$q_1$};

\path
(A) edge [bend left ] node [above]  {1} (B)
(B) edge [loop above] node [above] {0} (B);
\end{tikzpicture}

==> tikz/omega_graph_ab.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
semithick]
%\tikzstyle{every state}=[fill=red,draw=none,text=white]

\node[state] (A)                    {X};
\node[state] (B) [right of=A] {Y};

\path
(A) edge [bend left] node [above]  {a} (B);
\path
(B) edge [bend left] node [below]  {b} (A);
\end{tikzpicture}
